Ivy-Fake: A Unified Explainable Framework and Benchmark for Image and Video AIGC Detection

The rapid development of Artificial Intelligence Generated Content (AIGC) techniques has enabled the creation of high-quality synthetic content, but it also raises significant security concerns. Current detection methods face two major limitations: (1) the lack of multidimensional explainable datasets for generated images and videos. Existing open-source datasets (e.g., WildFake, GenVideo) rely on oversimplified binary annotations, which restrict the explainability and trustworthiness of trained detectors. (2) Prior MLLM-based forgery detectors (e.g., FakeVLM) exhibit insufficiently fine-grained interpretability in their step-by-step reasoning, which hinders reliable localization and explanation. To address these challenges, we introduce Ivy-Fake, the first large-scale multimodal benchmark for explainable AIGC detection. It consists of over 106K richly annotated training samples (images and videos) and 5,000 manually verified evaluation examples, sourced from multiple generative models and real world datasets through a carefully designed pipeline to ensure both diversity and quality. Furthermore, we propose Ivy-xDetector, a reinforcement learning model based on Group Relative Policy Optimization (GRPO), capable of producing explainable reasoning chains and achieving robust performance across multiple synthetic content detection benchmarks. Extensive experiments demonstrate the superiority of our dataset and confirm the effectiveness of our approach. Notably, our method improves performance on GenImage from 86.88% to 96.32%, surpassing prior state-of-the-art methods by a clear margin.

==> readme.tex <==
---
language: 
  - en
tags:
- AIGC Detection
- Fake Image and Video Detection
datasets:
- AI-Safeguard/Ivy-Fake
base_model: "Qwen/Qwen2.5-VL-3B-Instruct"
---

# [ICMR 2026]Ivy-Fake: A Unified Explainable Framework and Benchmark for Image and Video AIGC Detection

<div align="center">

<h4>
<a href="https://arxiv.org/abs/2506.00979">�� arXiv Paper</a> &nbsp; 
<a href="https://pi3ai.github.io/IvyFake">�� Project Page</a> &nbsp; 
<a href="https://huggingface.co/AI-Safeguard/Ivy-Fake">�� Hugging Face Models</a>
<a href="https://huggingface.co/datasets/AI-Safeguard/Ivy-Fake">�� Hugging Face Datasets</a>
</h4>

</div>


## News

- �� `2026.4` Our paper has been accepted by ICMR 2026.
- �� `2026.2` We release our models ��[**Ivy-xDetector**](https://huggingface.co/AI-Safeguard/Ivy-Fake) for **AI-generated image and video detection**������!
- �� `2025.12` The [**Ivy-Fake Dataset**](https://huggingface.co/datasets/AI-Safeguard/Ivy-Fake) is released.
- �� `2025.5` We release the [**Arxiv**](https://arxiv.org/abs/2506.00979)

## �� Getting Started

# How to Get Started with the Model

The following snippet demonstrates how to perform inference using our model with the `transformers` library.

```python
import torch
from transformers import Qwen2_5_VLForConditionalGeneration, AutoProcessor
from qwen_vl_utils import process_vision_info

# Initialize Model and Processor
model_id = "AI-Safeguard/Ivy-Fake"
model = Qwen2_5_VLForConditionalGeneration.from_pretrained(
    model_id,
    torch_dtype=torch.bfloat16,
    attn_implementation="flash_attention_2",
    device_map="auto",
)
processor = AutoProcessor.from_pretrained(model_id)

# Define the Detection Prompt
messages = [
    {
        "role": "system",
        "content": "You are an AI-generated content detector. Classify the media as real or fake. Provide reasoning inside <think>...</think> tags. End with exactly one word—real or fake—wrapped in <conclusion>...</conclusion>."
    },
    {
        "role": "user",
        "content": [
            {
                "type": "image",
                "image": "https://path-to-your-image.jpg", # Replace with your media path
            },
            {"type": "text", "text": "Is this image real or fake?"},
        ],
    }
]

# Preparation for Inference
text = processor.apply_chat_template(messages, tokenize=False, add_generation_prompt=True)
image_inputs, video_inputs = process_vision_info(messages)
inputs = processor(
    text=[text],
    images=image_inputs,
    videos=video_inputs,
    padding=True,
    return_tensors="pt",
).to("cuda")

# Generation
generated_ids = model.generate(**inputs, max_new_tokens=2048, do_sample=False)
generated_ids_trimmed = [
    out_ids[len(in_ids) :] for in_ids, out_ids in zip(inputs.input_ids, generated_ids)
]
output_text = processor.batch_decode(
    generated_ids_trimmed, skip_special_tokens=True, clean_up_tokenization_spaces=False
)

print(output_text[0])
```

---

## Citation

If you find Ivy-Fake or IVY-XDETECTOR useful in your research, please cite:

```bibtex
@article{jiang2025ivy,
  title={Ivy-fake: A unified explainable framework and benchmark for image and video aigc detection},
  author={Jiang, Changjiang and Dong, Wenhui and Zhang, Zhonghao and Si, Chenyang and Yu, Fengchang and Peng, Wei and Yuan, Xinbin and Bi, Yifei and Zhao, Ming and Zhou, Zian and others},
  journal={arXiv preprint arXiv:2506.00979},
  year={2025}
}
```
